Semantic Identifiers and DNS Names for IoT

In this paper, we propose a scheme for representing semantic metadata of IoT devices in compact identifiers and DNS names to enable simple discovery and search with standard DNS servers. Our scheme defines a binary identifier as a sequence of bits: a Context to use and several bits of fields corresponding to semantic properties specific to the Context. The bit string is then encoded as base32 characters and registered in DNS. Furthermore, we use the compact semantic DNS names to offer support for search and discovery. We propose to take advantage of the DNS system as the basic functionality for querying and discovery of semantic properties related to IoT devices. We have defined three specific Contexts for hierarchical semantic properties as well as logical and geographical locations. For this last part, we have developed two prototypes for managing geo-identifiers in LoRa networks, one based on Node and the Redis in-memory database, the other one based on the CoreDNS server.

==> figs/dnsdb_workflow.tex <==
\begin{tikzpicture}
  \node[rectangle, draw] (app) at (0, 0){Application};
  \node[rectangle, draw] (ns) at (3, 0){Network Server};
  \node[rectangle, draw] (dev) at (6, 0){Device};
  \node[rectangle, draw] (dns) at (2, 1){DNS-SD};

  \draw[->] (app) -- (dns);
  \draw[->] (dns) -- (app);
  \draw[->] (app) -- (ns);
  \draw[->] (ns) -- (dev);
\end{tikzpicture}

